Optimized Bayesian Framework for Inverse Heat Transfer Problems Using Reduced Order Methods

A stochastic inverse heat transfer problem is formulated to infer the transient heat flux, treated as an unknown Neumann boundary condition. Therefore, an Ensemble-based Simultaneous Input and State Filtering as a Data Assimilation technique is utilized for simultaneous temperature distribution prediction and heat flux estimation. This approach is incorporated with Radial Basis Functions not only to lessen the size of unknown inputs but also to mitigate the computational burden of this technique. The procedure applies to the specific case of a mold used in Continuous Casting machinery, and it is based on the sequential availability of temperature provided by thermocouples inside the mold. Our research represents a significant contribution to achieving probabilistic boundary condition estimation in real-time handling with noisy measurements and errors in the model. We additionally demonstrate the procedure's dependence on some hyperparameters that are not documented in the existing literature. Accurate real-time prediction of the heat flux is imperative for the smooth operation of Continuous Casting machinery at the boundary region where the Continuous Casting mold and the molten steel meet which is not also physically measurable. Thus, this paves the way for efficient real-time monitoring and control, which is critical for preventing caster shutdowns.

==> sections/Nomenclature.tex <==
\begin{flushleft}
    \Large\bfseries Nomenclature
\end{flushleft}
\begin{tabular}{@{}p{2cm}l@{}}
    CC  & Continuous Casting \\
    DA  & Data Assimilation \\
    EnKF  & Ensemble Kalman Filter \\
    EnSISF  & Ensemble-based Simultaneous Input and State Filtering \\
    EnKF-wDF  & EnSISSF with direct feedthrough (EnSISF-wDF)\\
    FOM  & Full Order Model \\
    HF  & Heat Flux \\
    IHTP  & Inverse Heat Transfer Problem \\
    PDEs  & Partial Differential Equations \\
    RBFs  & Radial Basis Functions \\
    UQ  & Uncertainty Quantification \\
     \quad &  \textcolor{red}{Add, Double check and modify}
\end{tabular}



